Randomness In Neural Network Training: Characterizing The Impact of Tooling

The quest for determinism in machine learning has disproportionately focused on characterizing the impact of noise introduced by algorithmic design choices. In this work, we address a less well understood and studied question: how does our choice of tooling introduce randomness to deep neural network training. We conduct large scale experiments across different types of hardware, accelerators, state of art networks, and open-source datasets, to characterize how tooling choices contribute to the level of non-determinism in a system, the impact of said non-determinism, and the cost of eliminating different sources of noise. Our findings are surprising, and suggest that the impact of non-determinism in nuanced. While top-line metrics such as top-1 accuracy are not noticeably impacted, model performance on certain parts of the data distribution is far more sensitive to the introduction of randomness. Our results suggest that deterministic tooling is critical for AI safety. However, we also find that the cost of ensuring determinism varies dramatically between neural network architectures and hardware types, e.g., with overhead up to $746\%$, $241\%$, and $196\%$ on a spectrum of widely used GPU accelerator architectures, relative to non-deterministic training. The source code used in this paper is available at https://github.com/usyd-fsalab/NeuralNetworkRandomness.

==> Sections/abstract.tex <==
\begin{abstract}
  There has been considerable investment in software and hardware design that preserves determinism in deep neural network training. This focus has been motivated by ensuring reproducibility of machine learning results and eliminating any noise independent of algorithm performance. However, the justification for determinism as a desiderata in machine learning research has occurred in the absence of any comprehensive characterization of the cost or impact of non-determinism. In this work, we conduct large scale experiments across widely used architecture and machine learning models to characterize both what contributes to the amount of non-determinism in a system, the impact of said non-determinims, and the cost of eliminating noise.
\end{abstract}

==> Sections/background.tex <==
\section{Background and Related Work}
\label{sec:background}

With the prosperity of deep learning community, solving sophisticated, non-convex optimization problems on high-dimensional input space using deep neural networks (DNNs) have become one of the most essential approach in the field of, for example, Image Classification \cite{alexnet,resnet}, Machine Translation \cite{gnmt,transformer}, and Object Detection \cite{fpn}. Neural Network training is stochastic process featured by stochastic mini-batch gradient decent, randomized weights initialization, non-deterministic computation in deep learning frameworks \cite{tensorflow,pytorch}, vendor libraries \cite{cudnn}, and intrinsic computation pattern in GPUs. 

Stochasticity in deep neural network training effectively explores diversified function space \cite{ensemble}, make the possibility for optimization algorithms to find better, well-calibrated solution with multiple trials. However, on the other hand, stochasticity is making result inconsistent between end-runs, thus hindering the reproducibility, debuggability, and reliability in safety critical applications. Over the past few years, a few work have been proposed to characterize and tackle the stochasticity in the deep neural network training procedure. \cite{pandoindeeplearning} reveals the lack of awareness in the research community to the stochasticity in deep learning system, as well as the awareness to perform multiple training runs to quantify the variance of their deep learning approaches and justify the improvement over baseline is statistically significant enough. \cite{impactofnondeterminismrl} proposed deterministic deep Q-Learning algorithm and points out that even single source non-determinism can result in large difference between end-runs in deep reinforcement learning models. \cite{drlmatters} trying to characterize the challenge proposed by reproducibility, experimental techniques, and reporting procedure. The authors shows the variability in reported metrics, and proposed guidelines to make deep reinforcement learning model more reproducible. 

Besides the algorithmic level noise in model training procedure, another source of noise is from implementation level that introduced by deep learning frameworks, vendor libraries, and GPUs. The profiling based heuristic computational kernel tuning, stochastic threads scheduling over massive parallelism combined with non associative floating point computation brings the designs that trade deterministic for performance. In the computer architecture research community, researchers have proposed several deterministic GPU architectures \cite{gpudet,dab} to boost the reproducibility and debuggability of GPU workloads. However, despite the significant performance overhead imposed by determinism, one cannot utilize the merit of deterministic GPU architecture in real world applications without first manufacture it, which is far from the out-of-the box utilization expected by the  deep learning community.

To this end, in the rush to mitigating or eliminating noise in deep learning system, a natural question that have not been discussed thoroughly would be: "What is the impact of noise? Does the impact is detrimental enough that worth paying all the efforts on controlling it?". To address this, We weight the benefit of controlling algorithmic and implementation noise in section \ref{sec}. We formulate this categorization not only because align with existing deep learning technology stack hierarchy, more importantly, controlling implementation noise comes with non-negligible performance overhead. As such we cannot eliminate all source of noise without sufficient justification.

\cite{risnotr} separating the notation of reproducibility from replicability. The author holds the point that reproducibility is desirable while replicability is not. Intuitively one do not have to fully control all sources of noises in the context of reproducibility. Interestingly, we argue that, even  top-line metric is reproducible, single source of noise may introduce disproportionately high variance and errors on a small subset of examples due to the biases in feature representation \ref{sec}. Therefore, enforce reproducibility fully control noise is critical in scenarios that sensitive to per-class accuracy and/or prevent involving unpredictable high accuracy variance gender and race basis.


==> Sections/checklist.tex <==

\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Sections/experiment.tex <==
\section{Experiment}
\label{sec:experiment}

Methodology
We measure the difference between models according to two core metrics:
\begin{enumerate}
    \item L2 norm - we compute the normalized L2 norm between weights.
    \item Churn - Disagreement between the predictions of multiple models It refers to the fraction of test examples where the predictions of two models disagree.
Standard deviation in test-set accuracy - percentage of variance in test-set accuracy explained by implementation noise vs algorithmic noise.
\end{enumerate}




==> Sections/intro.tex <==
\section{Introduction}

There has been a considerable amount of investment in hardware and software designed to eliminate stochasticity from deep neural network training. The quest to eliminate noise in ML has focused considerable attention on the design of hardware and software that is deterministic. A deterministic setting allows for the replicability of an experiment, here defined as \textit{ensuring the same result given the same inputs and hardware}. In the field of machine learning, the urgency to remove noise is often motivated by 1) concerns of reproducibility, 2) having full experimental control and/or 3) the need to precisely audit AI behavior in safety critical applications.

The quest for non-determinism has spurred new research on GPU designs which are deterministic \cite{gpudet,dab} and software patches that ensure determinism \cite{determinismindeeplearning}. Popular libraries such as Tensorflow, Jax and Pytorch have invested in deterministic modes, and new .  


However, in our rush to eliminate noise from ML systems, we seem to have skipped a crucial step -- characterizing the impact of the problem or the cost of controlling noise in the system. Understanding the origins of noise in ML systems is critical in order to weigh the benefits of controlling for implementation and algorithmic noise. Determinism comes at a non-trivial cost as it often imposes considerable latency overhead on training.

In this work, we conduct large scale experiments across widely used architecture and machine learning models to characterize both what contributes to the amount of non-determinism in a system, the impact of said non-determinims, and the cost of eliminating noise. Our results are surprising, and suggests that a more nuanced view of non-determinism is merited.



% We introduce a taxonomy to more precisely understand the contribution of both implementation choices (arising from the choice of hardware and software) and algorithmic choices (resulting from choices made in deep learning algorithm design) to the overall level of noise in an ML system. In large scale experiments, we evaluate and characterize noise across multiple datasets, models and types of hardware. Our results are surprising from the perspective of noise impact, interaction and accumulation of multiple noise sources as well as the best practice of enforcing determinism with minimum overhead.
Our contributions can be enumerated as follows:
\begin{itemize}
    \item We reveal the lack of attention of the impact of non-determinism on per-class accuracy critical workloads. The per-class uncertainty is unproportionately magnified even on datasets and models that are unsensible to noise.
    \item Noise introduced by algorithmic choices like batching size or random shuffling dominate overall system noise.
   \item Paradoxically, in some cases, implementation noise leads to lower variance between end-runs. Implementation noise dose not have negative impact to top-line metrics, surprisingly, in some cases, implementation noise is making outcomes more efficient and predictable. 
    \item We demonstrate that fully deterministic does not means noise-free. 
    \item We find that controlling for implementation noise (the noise introduced by deep learning framework and GPU hardware) poses significant overheads to model training procedure -- up to 123\% overhead in the execution time of GPU. To alleviate this, we further propose the network architecture design guidance targeting minimum training speed degradation for future researchers and engineers who are working on developing reproducible deep neural networks.
\end{itemize}
 




==> Sections/nondeterminism.tex <==
\subsection{Non-Determinism in Deep Neural Network Training}
\subsubsection{Source of Non-Determinism}

Implementation noise - implementation noise is the variance introduced by both hardware and software sources of non-determinism. 

1.Atomic [[donglin to add details]] 
2.Buffer [[donglin to add details]]
3.Precision [[donling to add details]]


Noise Categorization
1. Implementation noise
2. Algorithmic Noise
